Generating Synthetic Handwritten Historical Documents With OCR Constrained GANs

We present a framework to generate synthetic historical documents with precise ground truth using nothing more than a collection of unlabeled historical images. Obtaining large labeled datasets is often the limiting factor to effectively use supervised deep learning methods for Document Image Analysis (DIA). Prior approaches towards synthetic data generation either require expertise or result in poor accuracy in the synthetic documents. To achieve high precision transformations without requiring expertise, we tackle the problem in two steps. First, we create template documents with user-specified content and structure. Second, we transfer the style of a collection of unlabeled historical images to these template documents while preserving their text and layout. We evaluate the use of our synthetic historical documents in a pre-training setting and find that we outperform the baselines (randomly initialized and pre-trained). Additionally, with visual examples, we demonstrate a high-quality synthesis that makes it possible to generate large labeled historical document datasets with precise ground truth.

==> section/related_work.tex <==
\section{Related Work}
\label{toc:related_Work}

%\begin{figure}[t]
%\centering
%
%\subfloat[Book 1]{
%\includegraphics[width=.45\columnwidth,  height=4cm]{hba/plutarchus-1-100-page-033.jpg}\label{fig:TODO}}
%\hfil
%\subfloat[Book 2]{
%\includegraphics[width=.45\columnwidth, height=4cm]{hba/justinien-pages-1-232-006.jpg}\label{fig:TODO}}
%\vfil
%\subfloat[Book 3]{
%\includegraphics[width=.45\columnwidth, height=4cm]{hba/girart-014.jpg}\label{fig:TODO}}
%\hfil
%\subfloat[Book 4]{
%\includegraphics[width=.45\columnwidth, height=4cm]{hba/cy-1-162-020.jpg}\label{fig:TODO}}
%\vfil
%\subfloat[Book 5]{
%\includegraphics[width=.45\columnwidth, height=4cm]{hba/voyage-018.jpg}\label{fig:TODO}}
%\hfil
%\subfloat[Book 6]{
%\includegraphics[width=.45\columnwidth, height=4cm]{hba/chartreuse-009.jpg}\label{fig:TODO}}
%
%\caption{
%Sample pages of each historical book used from the HBA 1.0 dataset. 
%(a) Book 1: ``Plutarchus, Vitae illustrium virorum". 
%(b) Book 2: ``Justinien, Institutes". 
%(c) Book 3: ``Girart d'Amiens, Meliacin ou le Cheval de fust". 
%(d) Book 4: ``Cy, commencent le Proc\`{e}s de Belial \`{a} l'encontre de Jh\'{e}sus". 
%(e) Book 5: ``Voyage pittoresque de la Gr\`{e}ce".
%(f) Book 6: ``La Chartreuse de Parme"
%}
%\label{fig:hba_samples}
%\end{figure}

% In this section, we briefly summarize the relevant related work to our scenario.
This section briefly outlines the research most closely related to our work. 

\subsection{Document Image Annotation and Synthesis}

The process of creating ground truth for labeled datasets is often
time-consuming and challenging.
To ease this process, several software tools have been created to assist
researchers in the annotation process.
Groundskeeper~\cite{yanikoglu1995complete},
TrueViz~\cite{haleeArchitectureTrueVizGroundTRUth2003} and
PerfectDoc~\cite{yacoubPerfectDocGroundTruthing2005} are some examples of ground
truthing tools that allow users to annotate documents in terms of regions,
lines, words, character glyphs and reading order.
These tools do not incorporate automation, and rely on the user to annotate the
entire document.

Other tools incorporate automated or semi-automated methods in addition to manual
methods to assist the user with annotations.
Aletheia~\cite{clausnerAletheiaAdvancedDocument2011} and 
DIVAnnotation~\cite{seuretSemiautomatizedModularAnnotation2018} assist the user
with methods to shrink bounding boxes, generate outlines with smearing-based
techniques, component selection, binarization and text-line extraction methods.
GraphManuScribble~\cite{garzCreatingGroundTruth2016} and the approach of Kassis
and El-Sana~\cite{kassisScribbleBasedInteractive2016} use graph-based approaches
provide the user with an interface to perform page layout segmentation by
scribbling on the page to isolate various components. 

Another approach towards creating labeled datasets involves the creation of
synthetic documents and their corresponding ground truth.
Baird~\cite{bairdDocumentImageDefect1992}, Kieu et
al.~\cite{kieuCharacterDegradationModel2012} and Seuret et
al~\cite{seuretGradientdomainDegradationsImproving2015a} focus on degrading real
document images using defect models to augment datasets.
Other tools such as DocEmul~\cite{capobiancoDocEmulToolkitGenerate2017a} and
DocCreator~\cite{journetDocCreatorNewSoftware2017a} aim to create synthetic
document images using a combination of user-specified structure, background
extraction, degradation methods, and other data augmentation approaches.  
However, such approaches still require human expertise in designing appropriate
pipelines to generate realistic documents. 

% TODO: decide if this stays in related work or in intro
%Conditioned on the success of deep learning based synthesis methods (see
%Section~\ref{TODO}), several learning-based approaches have been proposed
%recently to reduce the requirement of human-expertise.
%Atarsaikhan et al.~\cite{atarsaikhanNeuralFontStyle2017a} successfully generated
%individual characters in various font styles using the Neural Style Transfer
%approach~\cite{Gatys_2016_CVPR}, however they do not synthesis any larger
%components such as words or lines.
%Pondenkandath et al.~\cite{pondenkandathHistoricalDocumentSynthesis2019a}
%utilize the CycleGAN framework~\cite{zhuUnpairedImagetoimageTranslation2017} to
%learn a mapping from modern electronic documents that specify the style and
%content to documents that resemble the style of a given collection of historical
%manuscriuse a pts.
%While the documents produced by this method match the overall style and look of
%the target documents, the underconstrained nature of the CycleGAN approach
%results in a mismatch in the textual content between the source document and the
%synthetic document.
%Tensmeyer~\cite{tensmeyerGeneratingRealisticBinarization2019} also utilize the
%CycleGAN framework in conjunction with background extraction and document
%degradation methods to synthesize binarization masks.
%Guan et al.~\cite{guanImprovingHandwrittenOCR2020} use style-conditioned
%\acp{GAN} to transform a skeletonized handwriting sample to a realistic image,
%however their approach requires matched datasets of skeletonized and realistic
%images which are non-trivial to generate.
%Kang et al.~\cite{kangGANwritingContentConditionedGeneration2020} use a style
%conditioned \acp{GAN} approach to generate handwritten text of fixed length that
%match the style characteristics of a given writer.

%Davis et al.~\cite{davisTextStyleConditioned2020} use \acp{GAN} and autoencoders
%to transform text and style vectors to synthetic handwritten text, however their
%approach relies on transcribed datasets. 
%~
%Alternatively, other tools are more focused on synthesising artificial documents
%(and their corresponding ground truth) that satisfy required constraints.
%~
%Aletheia~\cite{clausnerAletheiaAdvancedDocument2011} - ground truthing tool with
%automated and semi-automated methods of annotation datasets at a large scale,
%support for features like bounding box shrinking, smearing based outline
%generation, component selection 
%~
%DIVAnnotation~\cite{seuretSemiautomatizedModularAnnotation2018} - manual ground
%truthing with support for automated methods like binarization, text-line
%bounding box extraction methods, seam carving, polygonalization methods, etc
%~
%Groundskeeper~\cite{yanikogluPINKPANTHERCOMPLETE1998} - create page segmentation
%GT manually with GUI tool using drawn zones and tags. nice features include
%polygonal regions, flexible metadata, reading order support
%~
%TrueViz~\cite{haleeArchitectureTrueVizGroundTRUth2003} - cross-platform GUI tool
%used for annotation rectangular regions, lines, words, characters and reading
%order. manual. limited support for complex layouts due to only supporting
%rectangular regions. 
%~
%PerfectDoc~\cite{yacoubPerfectDocGroundTruthing2005} - mainly correction tool,
%but with support for ground truthing. multi-page reading order, bounding box
%regions, only manual

\subsection{Image-to-Image Translation}

The goal of an image-to-image translation process is to translate a given image
to another image.
These transformations can work on complete images, transforming them between
different domains or depictions (drawing to photo-realistic images) or on
objects within the images (horses to zebras). 
Such image translation problems can be viewed as an image conditioned
synthesis process~\cite{Isola_2017_CVPR}, with applications towards style
transfer~\cite{Chang_2018_CVPR},
super-resolution~\cite{jiangEdgeEnhancedGANRemote2019},
colorization~\cite{nazeriImageColorizationUsing2018} and
depth-estimation~\cite{Zheng_2018_ECCV}.

Some approaches towards image-to-image translation rely on paired datasets with
matched image pairs from both the source and target domains, while other
approaches work with unmatched collections of images from the two different
domains. 
Using paired datasets, Isola et
al.~\cite{isolaImagetoimageTranslationConditional2017} used an
image-conditioned \ac{GAN} approach (Pix2Pix) to learn a mapping from input images to
output images (for e.g., overhead satellite view to map view). 
% TODO add more paired dataset synthesis examples 

Approaches towards working with unpaired datasets can be categorized into
four main categories following the scheme described by Huang et
al.~\cite{huangIntroductionImageSynthesis2018}.
These approaches use:
\begin{itemize}
\item Cycle consistency loss with bi-directional
  reconstruction~\cite{zhuUnpairedImagetoimageTranslation2017,Yi_2017_ICCV,kimLearningDiscoverCrossdomain2017}
\item Pair-wise distance constraint loss~\cite{benaimOnesidedUnsupervisedDomain2017}
\item Task specific auxiliary classifier~\cite{Bousmalis_2017_CVPR}
\item \acp{VAE} with shared-weight generators~\cite{liuUnsupervisedImagetoimageTranslation2017}
\end{itemize}

In this work, we use the CycleGAN approach outlined by Zhu et
al.~\cite{zhuUnpairedImagetoimageTranslation2017}, which extends the Pix2Pix
architecture with two additional networks and the cycle consistency loss.





==> section/related_work_bak.tex <==
\section{Background}

In this section, the related work to set the context of the paper and the theoretical background necessary to understand the paper are discussed.

\subsection{Transkribus}\label{subsec:transcribus}
Transkribus~\cite{kahle2017transkribus, jander2016handwritten} is an open-source tool for computer-aided transcription,  recognition, and retrieval of digitized historical documents. After a user uploads all his documents into the tool, the first task is to segment all words, either manually or automatically with the built-in layout analysis. In the second step, all allocated words are pre-transcribed with the \ac{HTR} of Transkribus and the user has to check each transcribed word and correct the mistakes made by the HTR. Afterwards the \ac{HTR} is trained on these words and the improvements of every unique training are synchronized with the global \ac{HTR} of Transkribus that allows all users to optimize it further. Since \ac{HTR} works the best on handwritten documents they are trained on, the automated transcription works significantly better on historical documents from popular and well-known authors or from time epochs with a lot of already transcribed documents in which only small errors have to be corrected later. On the other hand, completely unknown authors and time epochs will have mostly wrong word predictions and the transcription, therefore, has to be done mostly manually, which trains the \ac{HTR} for similar upcoming documents. 



\subsection{DocCreator}\label{subsec:doccreator}
DocCreator~\cite{journet2017doccreator, journet2017massive} is an open-source tool to generate synthetic ground truth documents. 

One possible approach is to generate this new synthetic document by composing it with a text given as an XML file that is pasted in the defined position with a desired background and font. 
For that, the tool offers to extract the background and the font from the given documents (the source domain)~\cite{journet2017doccreator}. 

A key difference between our approach and DocCreator is, that in the latter, no deep learning is involved in the synthesis process.
However, deep learning is used in DocCreator for the extraction of the characters to create a font, as
this is done with the \ac{OCR}~\cite{islam2017survey, arica2001overview} of Tesseract~\cite{smith2007overview, tesseractGit}.
Therefore, since DocCreator uses \ac{OCR} for font extraction, the automatic pre-assignment only works if the handwritten characters of the document are known to the OCR.

To create the font, the OCR of DocCreator analyzes the input of one (historical) document and tries to identify all characters that the document consists of. 
For every character the font contains, up to five (or more if configured) different recognized characters from the document are extracted and one of them is picked randomly every time a character is inserted with the font.
As far as we are aware, it is currently not possible to create a font with more than one image.
Errors in the recognition of one character can be fatal, as that would create a wrong ground truth for the characters in the training data, which can result in a malfunction of the deep learning algorithm and it may not be able to recover from the mistake~\cite{achille2018critical}. 

It is also possible to reconstruct the background from the desired document in a semi-automatic way. 
This is accomplished by first, applying a binarization on the documents from which the background should be constructed and then manually choosing a threshold that captures the complete text of the document but not the background.
 
It should be noted that the synthesized documents that are generated in the section "Generation with ground truth" have no new elements in them.
All characters, symbols as well as the background the new synthesized document contains are extracted components that were collected from the training data and just reordered according to the XML file specified for the synthesized document.  
\subsection{CycleGAN}\label{subsec:CycleGAN}

In 2014, the technolgy of \acp{GAN}~\cite{goodfellow2014generative} became popular, which are able to generate new, synthetic data that can pass for real data, and consist of a generator that generates the data and a discriminator who judes it. 
The task of the generator is to create an image out of a random input. 
The discriminator then receives the output of the generator as well as the real images that the generator is supposed to resemble. 
Based on the results of how the discriminator judged the images, a loss is determined to train both, the discriminator and the generator. 
If the discriminator predicted the nature of the majority of the images rightfully, the loss will be high for the generator low the discriminator is low and vice versa, if the discriminator was wrong in its prediction for the majority of the images. 
Since both, the generator and the discriminator, start their respective processes with no training, the first generated images of the generator are merely random pixels. The discriminator then guesses if these generated images are real or fake.
As the training progresses, they start to train each other by playing a minimax two-player game. 
The goal is to balance the training of both out and avoid that one gets better than the other, so they can learn from each other as long as possible.
In 2017, the successor of \acp{GAN}~\cite{goodfellow2014generative},  CycleGAN~\cite{zhu2017unpaired} was published, which can achieve image-to-image translation in an unsupervised manner.  
In image-to-image translation, the goal is to take an image of a source domain and convert it to resemble the style of the target domain. 
Like a normal \ac{GAN}, the CycleGAN tries to learn a mapping G from a source domain to target domain \( G : X \to Y \) with the adversarial loss, so that G(X) and Y are not distinguishable.
The main difference is, that the CycleGAN additionally learns the reversed mapping \(F: Y \to X \) with a cycle consistency loss that ensures that \( F(G(X)) = X \).
This cycle consistency enforces a strong connection between the domains, for the reason that a source image that is transformed to the target domain style has to contain enough information of the source to be able to be transformed back~\cite{zhu2017unpaired, almahairi2018augmented}. 
The third loss is the identity loss, which maps the source domain back to the source domain using F and should result in the same image: \( F(X) = X \). 
The identity loss helps CycleGAN to preserve the colors of the input images, that could otherwise be mapped into a completely different color spectrum~\cite{zhu2017unpaired}. 
